Hierarchical Decentralized Deep Reinforcement Learning Architecture for a Simulated Four-Legged Agent

Legged locomotion is widespread in nature and has inspired the design of current robots. The controller of these legged robots is often realized as one centralized instance. However, in nature, control of movement happens in a hierarchical and decentralized fashion. Introducing these biological design principles into robotic control systems has motivated this work. We tackle the question whether decentralized and hierarchical control is beneficial for legged robots and present a novel decentral, hierarchical architecture to control a simulated legged agent. Three different tasks varying in complexity are designed to benchmark five architectures (centralized, decentralized, hierarchical and two different combinations of hierarchical decentralized architectures). The results demonstrate that decentralizing the different levels of the hierarchical architectures facilitates learning of the agent, ensures more energy efficient movements as well as robustness towards new unseen environments. Furthermore, this comparison sheds light on the importance of modularity in hierarchical architectures to solve complex goal-directed tasks. We provide an open-source code implementation of our architecture (https://github.com/wzaielamri/hddrl).

==> edits_luca.tex <==
%<*abstract>
Principles found in nature have inspired technical developments for a long time. One example is the transition from driving robots that use wheels to walking robots on legs. %This enables robots to operate on nearly any surface. 
The controller for such robots, often resembles a centralized instance. However, in nature, control of movement happens in a hierarchical and decentralized way, 
%</abstract>

%<*ResultsIntro>
%</ResultsIntro>

%<*ResultsTask1>
Fig. \ref{fig:task1_averageRewad} (a) shows that the decentral architecture improves faster than the central architecture. This confirms the results of Schilling et al. \cite{schilling2021} how report a similar result, however, on the simpler task of moving forward instead of walking towards a set goal position.
In Fig. \ref{fig:task1_averageRewad} (b) it can be observed that the fully centralized architecture (\textcolor{cc}{1\_C\_C}) trains the slowest, whereas the fully decentralized architecture (\textcolor{dd}{1\_D\_D}) trains fastest. This indicates that the result of \cite{schilling2021} not only holds for a more complicated task, but also in this hierarchical model setup.
%</ResultsTask1>



%<*Table1Results>

%</Table1Results>Hm, jetzt ist das paper wieder 19 Seiten lang? Wie schalte ich deine Textversionen ein - irgendwas scheint hier nicht zu klappen. \newcommand{\alt}[3]{%

